Re-ReND: Real-time Rendering of NeRFs across Devices

This paper proposes a novel approach for rendering a pre-trained Neural Radiance Field (NeRF) in real-time on resource-constrained devices. We introduce Re-ReND, a method enabling Real-time Rendering of NeRFs across Devices. Re-ReND is designed to achieve real-time performance by converting the NeRF into a representation that can be efficiently processed by standard graphics pipelines. The proposed method distills the NeRF by extracting the learned density into a mesh, while the learned color information is factorized into a set of matrices that represent the scene's light field. Factorization implies the field is queried via inexpensive MLP-free matrix multiplications, while using a light field allows rendering a pixel by querying the field a single time-as opposed to hundreds of queries when employing a radiance field. Since the proposed representation can be implemented using a fragment shader, it can be directly integrated with standard rasterization frameworks. Our flexible implementation can render a NeRF in real-time with low memory requirements and on a wide range of resource-constrained devices, including mobiles and AR/VR headsets. Notably, we find that Re-ReND can achieve over a 2.6-fold increase in rendering speed versus the state-of-the-art without perceptible losses in quality.

==> imgs/6_ReflectanceMaps.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{imgs/ViewDirPpt.pdf}
    % \vspace{-0.5cm}
    \caption{
    \albert{remove}
   
    We show color as a function of elevation (y-axis) and azimuth (x-axis) for one point on the surface of the \textit{Materials} scene from the Synthetic dataset. 
    The first row is a pseudo-GT (extracted from MipNeRF), and subsequent rows are \methodname's output when varying the light field embedding dimension $D$. 
    }
    \vspace{-0.2cm}
    \label{fig:reflectance_maps}
\end{figure}

==> imgs/meshes.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{imgs/meshes.png}
    \caption{\albert{TODO}}
    \label{fig:Rendering}
\end{figure}

==> results/2_Resources_tb.tex <==
\begin{table}[t!]
\footnotesize
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l"lll"lll}\thickhline
Dataset      & \multicolumn{3}{c"}{Synthetic 360°} & \multicolumn{3}{c}{Unbounded 360°} \\
Method       & Ours    & SNeRG    & \shortstack{Mobile \\ NeRF}    & Ours  & SNeRG          & \shortstack{Mobile \\ NeRF}         \\\hline
GPU memory   &   239.3      &    5,707.3      &      538.38         &      397.5   &   3,388.3  &   1,063.0                 \\
Disk storage &   143.5      &    87.0      &         125.75      &    233.47   & 324.8  &    311.3               \\\thickhline
\end{tabular}
\caption{\textbf{Resources} – memory and disk storage (MB).}
\label{2_Resources}
\end{table}



==> results/3_Quantitative_tb.tex <==
\begin{table}[t!]
    \footnotesize
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{l"c|c|c"c|c|c}
        \thickhline
        & \multicolumn{3}{c"}{Synthetic 360°} & \multicolumn{3}{c}{Unbounded 360°} \\
        Method     & PSNR $\uparrow$      & SSIM  $\uparrow$     & LPIPS $\downarrow$     & PSNR  $\uparrow$    & SSIM  $\uparrow$     & LPIPS  $\downarrow$    \\\hline
        NeRF \cite{mildenhall2021nerf}      &   31.00  &    0.947        &     0.081       &   18.98         & 0.712        &  0.573     \\
        Mip-NeRF \cite{barron2021mipnerf}      &   33.09  &    0.961        &     0.043       &   -         & -        &  -     \\
        NeRF++  \cite{nerf++}   &   -             &   -             &    -            &   20.08  & 0.758 &  0.412     \\
        ADOP  \cite{ruckert2022adop}   &   -             &   -             &    -            &   23.53*  & - &  0.151*     \\\hline
        SNeRG   \cite{hedman2021snerg}  &    30.38        &   \best{0.950} & \best{0.050}     &   14.04           & 0.528 &  0.548     \\
        M-NeRF  \cite{chen2022mobilenerf}   &    \best{30.90} &   0.947         &   0.062         &   15.59           & 0.474        &  0.535     \\
        Ours       &    29.66        &   0.939         &  0.068         &   \best{17.91}    & \best{0.542}        &  \best{0.513}     \\
        % Ours$\bigstar$  &    28.67   &   0.927         &  0.079          &   18.31         & 0.561        &  0.488   \\
        \thickhline
    \end{tabular}
    % \vspace{-0.2cm}
    \caption{\textbf{Rendering Quality.} \sara{ADOP does not have truck scene but it has lighthouse???} In this table we present common measures of image quality for renderings from \methodname and several other non-real and real time NeRF pipelines on edge devices. We present this table as reference to show that \methodname achieves comparable image quality to more complex NeRF architectures, while being significantly faster. Note that we extract numbers directly from each corresponding paper, and omit values (with -) that were not originally reported by the methods. 
    }
    % \vspace{-0.2cm}
    \label{tab:3_Quantitative_tb}
\end{table}

==> results/4_Polygon_count_tb.tex <==
\begin{table}[t!]
    \footnotesize
    \centering
    \begin{tabular}{l"c|c"c|c}
        \thickhline
        & \multicolumn{2}{c"}{Synthetic 360°} & \multicolumn{2}{c}{Unbounded 360°}\\
        Method & M-NeRF & \methodname & M-NeRF & \methodname\\
        \thickhline
        Vertices & 494,289 &  \best{99,539} & 332,678 & \best{117,751}\\
        Faces    & 224,341 & \best{205,693} & 543,047 & \best{244,847}\\
        \thickhline                                            
    \end{tabular}
    % \vspace{-0.2cm}
    \caption{\textbf{Average Mesh Size.} We report the average number of vertices and triangle faces for meshes used by \methodname and MobileNeRF. 
    The meshes used by our method are substantially smaller than those used by MobileNeRF. %  is more economical in mesh requirements size.
    }
    % \vspace{-0.4cm}
    \label{tab:4_Polygon_count_tb}
\end{table}
